Self-Evolving Scientific Agent Designs Physically Reasoned White-Box Fluid Control

While neural networks excel in autonomous control, their black-box nature makes control decisions difficult to interpret and diagnose in dynamic fluids. Here, we show how self-evolving scientific agents can design explicit, neural-network-free white-box controllers by iteratively interpreting simulation evidence, accumulating control knowledge and refining controller code. We demonstrate this approach on an underactuated two-joint swimmer navigating unsteady flows via joint angular accelerations. Starting from a target-blind propulsive controller, the agent gradually constructs key mechanisms, including travelling-wave propulsion, body-frame guidance, phase-selective steering, redirect bursts and adaptive relief. The resulting controllers reach targets and generalize across changes in target position, wake geometry, cylinder count, and inflow speed without revision. Moreover, 2D control priors transfer successfully to accelerate 3D adaptation. Our work demonstrates that self-evolving agents can autonomously design physically reasoned and generalizable white-box fluid control, showing a promising paradigm beyond traditional reinforcement learning and black-box neural network control.

==> sections/00_preamble.tex <==
% sn-jnl supplies the publisher's page geometry; the Supplementary keeps its own.
\makeatletter
\@ifpackageloaded{geometry}{}{\usepackage[margin=1in]{geometry}}
\makeatother
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{xcolor}
\makeatletter
\@ifpackageloaded{natbib}{\setcitestyle{super}}{%
  \usepackage[numbers,sort&compress,super]{natbib}}
\makeatother
\usepackage{url}
\usepackage{xurl}
\makeatletter
\@ifpackageloaded{hyperref}{%
  \hypersetup{hidelinks,hypertexnames=false}}{%
  \usepackage[hidelinks,hypertexnames=false]{hyperref}}
\makeatother
\usepackage{microtype}
\usepackage{placeins}
\usepackage{array}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{float}
\usepackage[breakable]{tcolorbox}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\graphicspath{{./}}
\setlength{\textfloatsep}{8pt plus 2pt minus 2pt}
\setlength{\floatsep}{8pt plus 2pt minus 2pt}
\setlength{\intextsep}{6pt plus 2pt minus 2pt}

\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{8pt plus 1fil}
\setlength{\@fpbot}{0pt plus 1fil}
\makeatother

